A Thorough Comparison of Cross-Encoders and LLMs for Reranking SPLADE

We present a comparative study between cross-encoder and LLMs rerankers in the context of re-ranking effective SPLADE retrievers. We conduct a large evaluation on TREC Deep Learning datasets and out-of-domain datasets such as BEIR and LoTTE. In the first set of experiments, we show how cross-encoder rerankers are hard to distinguish when it comes to re-rerank SPLADE on MS MARCO. Observations shift in the out-of-domain scenario, where both the type of model and the number of documents to re-rank have an impact on effectiveness. Then, we focus on listwise rerankers based on Large Language Models -- especially GPT-4. While GPT-4 demonstrates impressive (zero-shot) performance, we show that traditional cross-encoders remain very competitive. Overall, our findings aim to to provide a more nuanced perspective on the recent excitement surrounding LLM-based re-rankers -- by positioning them as another factor to consider in balancing effectiveness and efficiency in search systems.

==> table/bm25.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering
\caption{
Evaluation (nDCG@10) of GPT4 with bm25 
}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{clccccccccc}
\toprule
& \textbf{topk}
& \textbf{length}
& \textbf{DL19}
& \textbf{DL20}
& \textbf{DLHARD}
& \textbf{DL21} 
& \textbf{DL22} 
& \textbf{Trec-covid} \\
\midrule
baseline &  &  & &\\
\midrule
a & 20  &  -1& 64.79&\\
  & 50   &  -1 &71.11/71.34\\
  & 75   &   -1 & 0.7430 \\ 
  &  100 &  -1  & 74.06 ? /0.7370/ 0.7367\\
128K&  100 &  -1  & 72.28\\
\bottomrule
\end{tabular}
}
\label{tab:bm25}
\end{table*}

% dl19   75  -> 90    100 -> 49   50 ->-1


==> table/gpt4.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering
\caption{
Evaluation (nDCG@10) from the litterature
}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{clccccccccccc}
\toprule
& \textbf{ref}
& \textbf{retriever}
& \textbf{topk}
& \textbf{window mechanism}
& \textbf{DL19}
& \textbf{DL20}
& \textbf{DLHARD}
& \textbf{DL21} 
& \textbf{DL22} 
& \textbf{Trec-covid} 
& \textbf{Trec-news} & NovelEval\\
\midrule
& Splade ed++  && & & 73.08 &71.95 & & 68.46&57.05   & 72.74 &  41.52 \\
%a & rankgpt &bm25&100 & window& 75.59&70.56\\
%b & jimmy  &bm25& 100& PSC& 75.66& 71.00\\
%b & jimmy  &bm25& 100& simple& 75.00& 70.36\\
%b & jimmy  &bm25& 20& simple& 60.88 &57.7\\
b & jimmy  &splade ed++& 100& rankgpt&74.64(74.64)& 70.76(71.08)??\\
b & jimmy  &splade ed++& 100& rankgpt+psc&76.01& 75.14\\
b & jimmy  &splade ed++& 20& single& 73.21(73.36)& 71.97(73.63)\\
b & jimmy  &splade ed++& 20& single+psc& 76.87& 78.52\\  
   &  RangGPT4  &splade ed++  & 20/10? &&&&&&&87.92  & 53.27&90.45\\
  & rankzephyr &splade ed++& 100 &    20/10     &  78.16& 81.59&& 75.98& 66.92  & 85.35&50.60 & 89.34\\
  & rankzephyr $\rho$&splade ed++& 100 & 20/10        &  78.55& 82.55&& 76.88& 66.28  & 85.66&51.07\\
\bottomrule
\end{tabular}
}
\label{tab:gpt4}
\end{table*}

